Visual-Inertial Object Detection and Mapping

We present a method to populate an unknown environment with models of previously seen objects, placed in a Euclidean reference frame that is inferred causally and on-line using monocular video along with inertial sensors. The system we implement returns a sparse point cloud for the regions of the scene that are visible but not recognized as a previously seen object, and a detailed object model and its pose in the Euclidean frame otherwise. The system includes bottom-up and top-down components, whereby deep networks trained for detection provide likelihood scores for object hypotheses provided by a nonlinear filter, whose state serves as memory. Additional networks provide likelihood scores for edges, which complements detection networks trained to be invariant to small deformations. We test our algorithm on existing datasets, and also introduce the VISMA dataset, that provides ground truth pose, point-cloud map, and object models, along with time-stamped inertial measurements.

==> misc/MCMC_move_shape_id.tex <==
To identify the shape index online, we introduce an extra Metropolis-Hastings move. The transition kernel is a conditional distribution which concentrates at the current shape index and jumps to other indices equally likely:
\begin{equation}
T(k_t \rightarrow k_t')=
\begin{cases}
\mu &\quad k_t'=k_t\\
\frac{1-\mu}{N-1}  &\quad k_t' \neq k_t
\end{cases}
\label{eq-move}
\end{equation}
where $\mu \in (\frac{1-\mu}{N-1}, 1)$ and $N$ is the total number of shapes. Acceptance rate of the transition is:
\begin{equation}
\alpha_\text{MH}=\min\{
\frac{p(I_t|\{k', g\}_t)T(k_t'\rightarrow k_t)}
{p(I_t|\{k, g\}_t)T(k_t\rightarrow k_t')},
1\}.
\label{eq-accept}
\end{equation}

This does not work well and it seems stationary distribution of the transition kernel is NOT the proper posterior.


==> misc/verbose_paper_summary.tex <==
\section{Verbose Paper Notes}

\subsection{Feature Pyramid Network~\cite{lin2016fpn}}

\subsubsection{Abstract}
\begin{itemize}
\item top-down architecture with lateral connections is developed for building high-level semantic feature maps at all scales.

\item shows siginificant improvemnt as a {\it generic feature extractor} in various applications; state-of-the-art {\it single-model} results on COCO detection benchmark, outperforms COCO 2016 challenge winners
\end{itemize}

\subsubsection{Intro}
\begin{itemize}
\item Feature pyramids built upon image pyramids (featureized image pyramids) show superior accuracy in detection compared to single scale method, since all levels are semantically strong.

\item drawback: slow in inference and infeasible in training due to memory limitation; inconsistent train/test-time inference if only used in test time

\item featureized image pyramid not the ONLY way to achieve multi-scale: in-network pyramid feature hierarchy produces feature maps of different spatial resolutions, but large semantic gaps exist due to different depths

\item In this paper: combine low-res, semantically strong features with high-res, semantically weak features via a {\it top-down pathway and lateral connections}. Fig. 1(d) of the paper. Significance: in-network feature pyramids replaces featurized image pyramids without sacrificing representational power, speed, or memory. Difference from previous work: previous work aggregates feautre maps to the finest level on which prediction is made; FPN makes predictions on each feature map (then ?)
\end{itemize}

\subsubsection{Related}

Mentioned hand-crafted features before CNN becomes popular. Deep ConvNet-based object detector including OverFeat, R-CNN, SPPNet, Fast and Faster R-CNN with an emphasis on how scale is handled.

Finally touch other multi-layer methods including FCN (Fully Convolutional Net), Hypercolumn for segmentation. SSD and MS-CNN (?) for detection. Also mentioned recent works exploiting lateral/skip connections, e.g., U-Net. However, they do NOT make predictions independently at all levels and image pyramids are still needed to recognize objects across multiple scales.

\subsubsection{Structure}
\begin{itemize}
\item Bottom-up pathway. Use the last layer of each stage, which consists of several nearby feature maps of the same size, as reference set of feature maps, which are enriched to create pyramid. For ResNet, use the feature activations ouput by each stage's last residual block, denoted as $\{ C_2, C_3, C_4, C_5\}$ for conv2,3,4,5 outputs, whose strides are $\{ 4, 8, 16, 32\}$ w.r.t. the input image.

\item Top-down pathway. Upsample feature maps from higher pyramid levels to match the spatial size of lower level feature maps, merge both by lateral (same as skip?) connections/adding activiations. $3\times 3$ convolution is applied to each merged feature map to reduce alias introduced by upsampling. Call the generated feature maps $\{P_2, P_3, P_4, P_5 \}$.

\item Channels are fixed across all pyramid feature levels, which share  classifiers/regressors. ??? No-linearities in extra layers. ???

\end{itemize}

\subsubsection{App}
\begin{itemize}
\item Original RPN(Region Proposal Net): small subnetwork evaluated on dense $3\times 3$ sliding windows atop a single-scale conv feature map, performing object/non-object binary classification and bounding box regression. Realized by $3\times 3$ conv layer followed by two sibling $1\time 1$ conv for classification and regression, which are refered as a network {\it head}. The object/non-object criterion and bounding box regression target are defined w.r.t. a set of anchors (reference boxes), which are of multiple pre-defined scales and aspect ratios in order to cover objects of different shapes.

\item head = $3\times 3$ conv + two sibling $1\times 1$ conv for binary classification and box regression.

\item assign an RoI of width $w$ and height $h$ (w.r.t. the input image size) to the level $P_k$ of the feature pyramid by:
$$
k=\lfloor k_0 + \log_2(\sqrt{wh}/224) \rfloor.
$$

224 is the canonical ImageNet pre-training size, and $k_0$ is the target level on which an RoI with $w\times h=224^2$ is mapped into. In ResNet based Faster R-CNN, $C_4$ is used for detection. So here, set $k_0=4$. Example: For an $112\times 112$ RoI, it will be assigned to $k=3$.

\item Head: use RoI polling to extract $7\times 7$ features and attach two hidden 1024-dim FC+ReLU layers before final classification and box regression layers.

\end{itemize}

\subsection{ResNet}
A good paper for reviewing popular techniques in data augmentation, replace fc with fully convolutional layers and average pooling, etc.
\subsubsection{Intro}
\begin{itemize}
\item VGG and Highway networks reveal the crucial importance of network depth.
\item the problem of vanishing/exploding gradients make it hard to learn networks of increasing depth; normalized initialization and intermediate normalization layers enable networks with tens of layers to start converging for SGD with backpropagation.
\item even networks start converging, accuracy saturates and performances degrades rapidly with depth increasing; the degradation is NOT caused by overfitting, but indicates that not all systems are easy to optimize
\item Fig.2 shows a building block of residual learning: signal x goes to two or more weight layers connected by a ReLU, the original x is also added via so called ``shortcut connections'' to the output of the last weight layer, followed by another ReLU.
\end{itemize}

\subsubsection{Deep Residual Learning}
\begin{itemize}
\item instead of learning the original mapping $\mathcal H(x)$, a residual function $\mathcal F(x) \doteq \mathcal H(x)-x$ is learned
\item via the ``shortcut connections'', original signal $x$ is added to output of residual mapping $y=\mathcal F(x; \{W_i, b_i\})+x$
\item dimension of $\mathcal F(x)$ should match that of $x$; otherwise a linear projection $W_s$ is applied $y=\mathcal F(x; \{W_i, b_i\}) + W_s x$ to match size

\item Implementation details on ImageNet followed by origin of the technique
\begin{itemize}
\item Image resized with its shorter side randomly sampled in $[256, 480]$ for scale augmentation (VGG)
\item A $224\times 224$ crop is randomly sampled from an image or its horizontal flip, with per-pixel mean substracted (AlexNet)
\item Apply standard color augmentation (AlexNet)
\item Adopt batch normalization after each convolution and before activation (BN)
\item Initialize weights as in MSRinit (Delving deep into rectifiers)
\item SGD with a mini-batch size of 256, learning rate starts from 0.1 and is divided by 10 when the error plateaus, and the models are trained for up to 600k iterations.
\item Weight decay of 0.0001 and a momentum of 0.9.
\item Dropout is NOT used (practice in BN paper)
\end{itemize}

\item Deeper Bottleneck Architecture:
\begin{itemize}
\item Motivation: Reduce number of parameters, make training affordable.
\item Design: Replace the two layer building block with a three layer block wich each layer having filter size of $1\times 1$, $3\times 3$ and $1\times 1$. The first layer reduces the channels of feature maps (say from 256 to 64), while the last layer restores the channels (from 64 to 256), leaving the layer in between a bottleneck with smaller input/output dimensions.
\end{itemize}

\item Analysis of layer responses show that responses in ResNet are in general smaller than their plain network counterparts, which confirms the hypothesis that residual mappings approximate zero compared to non-residual mappings.
\end{itemize}

\subsubsection{Object detection}
\begin{itemize}
\item Adopt Faster R-CNN approach
\item conv1\_x to conv4\_x are shared by RPN and Fast R-CNN, RoI pooling is performed before conv5\_1. On the RoI-pooled feature, all layers of conv5\_x and up are adopted for each region, playing the roles of VGG-16's fc layers, which is used in the Faster R-CNN paper.
\item Final classficiation layer is replaced by two sibling layers: One for classification and one for box regression.
\item Parameters of BN layers are learned in pre-training (on ImageNet) and fixed during Faster R-CNN training.
\item Tricks:
\begin{itemize}
\item Box refinement: apply classification/regression on top of regressed boxes iteratively.
\item Global context: treat the whole image as an RoI region, from which a global context feature is extracted and concatenated to the original RoI feature. The concatenated feature is used for classification/regression.
\item Multi-scale testing: Build an image pyramid with the shorter side of length $s\in\{200, 400, 600, 800, 1000\}$; Select two adjacent scales from the pyramid according to ... RoI pooling and subsequent layers are performed on merged feature maps of the two selected layers.
\item Ensemble: use an ensemble for proposing regions and union of proposals are processed by an ensemble of per-region classifiers.
\end{itemize}
\end{itemize}

\subsection{Fast R-CNN}
\begin{itemize}

\item Overall structure:
\begin{itemize}
\item Input: an image and a set of object proposal.
\item Output: probability over $K$ classes plus a ``background'' class and four real-valued numbers for each of the $K$ object classes.
\item The whole image is processed with several conv and max pooling layers to produce a feature map. Then, for each object proposal a region of interest (RoI) pooling layer extracts a {\it fixed-length} feature vector from the feature map. Each feature vector is fed into a sequence of fully connected layers (fc) that finally branch into two sibling layers: one for classification and the other for box regression.
\end{itemize}

\item RoI pooling layer: use max pooling to convert features inside any valid RoI into a small feature map with a fixed spatial extent of $H\times W$ (RoI feature shape, not on the image plane). $H$ and $W$ are hyper-parameters that are independent of any particular RoI. Given a bounding box proposal and a feature map from a certain layer, we can locate a region in the feature map which corresponds to the given bounding box proposal. Such regions are called region of interest. Each RoI is defined by a four-tuple $(r, c, h, w)$ that specifies top-left corner $(r, c)$ and its height and width $(h, w)$. RoI max pooling works by dividing the $h\times w$ window into an $H\times W$ grid of sub-windows of approximate size $h/H \times w/W$ and then max-pool the values in each sub-window into the corresponding grid cell.

\item Initialization: take existing network trained for ImageNet classification and replace the last max-pooling layer with a RoI pooling layer, of which the parameters $H$ and $W$ are chosen to be compatible with the net's fc layer. The fc layer and softmax layer are replaced with two sibling layers for classification and regression. The network is modified to take objet proposals in addition to the image.

\item Hierarichical sampling of mini-batches: first randomly sample $N$ images and then randomly sample $R/N$ RoIs from each image. Though RoIs from the same image are potentially correlated, which violates the i.i.d. assumption of training data, there seems no practical issues in training.

\item Multi-task loss:
\begin{itemize}
\item The classification branch outputs discrete probability distribution over $K$ classes plus a background class: $p=(p_0, \cdots, p_K)$, which is given by the final fc layer followed by a softmax.
\item Regression branch outputs bounding-box regression offsets $t^k=(t_x^k, t_y^k, t_w^k, t_h^k)$ for each of the $K$ object class. Parametrization of $t^k$ follows R-CNN.
\item Each training RoI is labeled with a ground-truth class $u$ and a ground-truth bounding-box regression target $v$.
\begin{equation}
L(p, u, t^u, v) = L_{cls}(p, u) + \lambda \mathbbm{1}_{u \ge 1} L_{box}(t^u, v)
\end{equation}
where $L_{cls}(p,u) = -\log p_u$ is the cross entropy loss and
\begin{equation}
L_{loc}(t^u, v)= \sum_{i \in \{x, y, w, h\}} {\mathrm{smooth}_{L_1}(t_i^u-v_i)}
\end{equation}
in which
\begin{equation}
\mathrm{smooth}_{L_1}(x)=
\begin{cases}
0.5x^2  & \text{if} |x| < 1\\
|x|-0.5 & \text{otherwise}
\end{cases}
\end{equation}
\end{itemize}

\item Scale invariance: FIXME
\item truncated SVD for faster detection: FIXME

\end{itemize}

\subsection{Faster R-CNN}
\begin{itemize}
\item Bottleneck in two-stage object detection is proposal generation. For instance, Selective Search (SS) is an order of magnitude slower compared to Fast R-CNN, which is near real-time. Introduce Region Proposal Networks (RPN) which share convolutional layers with state-of-the-art object detection networks. Marginal cost for computing proposals is small by sharing weights.

\item On top of the conv features which are used in Fast R-CNN for detection, RPNs are constructed by adding two additional conv layers: one that encodes each conv map position into a short feature vector and a second that, at each conv map position, outputs an objectness score and regressed bounds for $k$ region proposals relative to various scales and aspect ratios at the location (typically $k=9$).

\item Training scheme: Alternate between fine-tuning for proposal generation (RPN) and fine-tuning for object detection (Fast R-CNN), while keeping the proposals fixed.

\item RPN
\begin{itemize}
\item Slide a mini-network over conv feature map from the last shared conv layer. The mini-network is fully connected to an $n\times n$ spatial window of the input conv feature map. Each sliding window is mapped to a lower-dimensional vector, which is then fed into two sibling fully-connected layers. The mini-network is implemented in a fully-convolutional fashion: an $n\times n$ conv layer is applied to the sliding window, followed by two sibling $1\times 1$ conv layers for classification and regression. ReLUs are applied to the output of the $n\times n$ conv layer.

\item Anchors: At each sliding-window location, predict $k$ region proposals, with each proposal containing $4$ real-valued numbers encoding the coordinates of the bounding box and $2$  scores denoting object/not-object. The $k$ proposals are parametrized relative to $k$ reference boxes, called anchors. Each anchor is centered at the sliding window in question, and is associated with a scale and aspect ratio. 3 scales and 3 aspect ratios, yielding $k=9$, are used.

\item Loss: contains two terms: one for binary classification and one for box regression. For classification, cross entropy is used. For box regression, smooth $L_1$ is used. Box coordinates are parametrized as follows: top-left corner is parametrized relative to the anchor in an affine transformation; width and height are parametrized relative to the anchor in log space.

\item Training procedure: Fast R-CNN needs fixed propsoals while training of RPN generates changing proposals.
\begin{itemize}
\item Fine-tune a network pre-trained on ImageNet as RPN.
\item Given proposals given by RPN, fine-tune another network pre-trained on ImageNet as Fast R-CNN.
\item Take and freeze weights of Fast R-CNN upto the last shared conv layer, fine tune the RPN specific branch.
\item Fine tune Fast R-CNN specific branch.
\item Alternate last two steps until convergence.
\end{itemize}
\end{itemize}

\item One-stage detection vs. two-stage proposal + detection. OverFeat paper proposes a detection method which basically regresses densly sampled bounding boxes. One can easily turn Fast R-CNN into a one-stage detection system by feeding Fast R-CNN densly sampled proposals, which shows degradation in performance. Also one-stage systems are slow since they operate densly on image.
{\it Why one-stage system performs worse? In theory, one-stage system should loss less information.}

\end{itemize}

\subsection{Mask R-CNN}
\begin{itemize}
\item Mask R-CNN extends Faster R-CNN by adding a branch for predicting segmentation masks on each RoI, in parallel with existing branch for classification and bounding box regression.
\item The mask branch is a small FCN applied to each RoI, which only adds a small computational overhead.
\item The core operation in Faster F-CNN is RoI pooling, which essentially performs coarse spatial quantization for feature extraction and thus introduces misaligment. A quantization-free layer, called RoIAlign, which faithfully preserves exact spatial locations, is proposed. The RoIAlign decouples mask and class prediction: a binary segmentation mask is predicted for each class independently. In contrast, previous segmentation network such as FCN couples segmentation and classification, which performs pooly for instance segmentation according to the authors' experiments.
\item RoIAlign operation: Instead of max-pooling features in a grid cell, features computed at four regularly sampled locations are aggregated, either via max or average-pooling, which themselves are computed via bilinear interpolation. Results are insentitive to exact sampling locations and number of sampling points, as long as no quantization is performed.
\item Mask representation: For each RoI, a total of $K$ $m\times m$ masks will be predicted, one for each class. The masks are real-valued and thresholding is needed to binarize them. In inference, only the most probable bounding box will be used, from which only the mask of the most probable class will be predicted. This differs training, but reduces inference time.
\item When backbone convolutional network is FPN (Feature Pyramid Network), the target level of feature map is found according to the proposal bounding box size, on top of which a network {\it head} for mask prediction is applied separately on each RoI.
\item Total loss $L=L_{cls} + L_{box} + L_{mask}$. $L_{mask}$ is only computed for the $k$-th class, where $k$ is the ground truth class label. Masks corresponding to the wrong class prediction do not contribute to the loss. $L_{mask}$ is defined as the average binary cross entropy.
\item Multinomial vs. Independent masks: One mask per class performs much better than multi-label prediction (usual way to do semantic segmentation), which suggests that {\it once the instance has been classified as whole (by the box branch), it is sufficient to predict a binary mask without convern for the categories}, which makes the model easier to train.
\item Class-specific vs. class-agnostic masks: Predicting one single mask for $K$ classes instead of one mask per class performs similarly, which further highlights {\it the effect of decoupling classification and segmentation}.
\end{itemize}




TOREAD:
\begin{enumerate}
\item Spatial Pyramid: SPPNet
\item Comprehensive evaluation: Speed/Accuracy trade-offs for modern convolutional object detectors.
\item Single-stage detectors: RetinaNet, SSD, YOLO?
\item Segmentation: DeepMask and SharpMask
\end{enumerate}

